SelfIE: Self-Interpretation of Large Language Model Embeddings

How do large language models (LLMs) obtain their answers? The ability to explain and control an LLM's reasoning process is key for reliability, transparency, and future model developments. We propose SelfIE (Self-Interpretation of Embeddings), a framework that enables LLMs to interpret their own embeddings in natural language by leveraging their ability to respond to inquiries about a given passage. Capable of interpreting open-world concepts in the hidden embeddings, SelfIE reveals LLM internal reasoning in cases such as making ethical decisions, internalizing prompt injection, and recalling harmful knowledge. SelfIE's text descriptions on hidden embeddings also open up new avenues to control LLM reasoning. We propose Supervised Control, which allows editing open-ended concepts while only requiring gradient computation of individual layer. We extend RLHF to hidden embeddings and propose Reinforcement Control that erases harmful knowledge in LLM without supervision targets.

==> theorybackup.tex <==


The residual connection allows us to decompose $\bm{y}_i$ (the output next token prediction at index $i$) as a geometric average over contributions of hidden embeddings from different layers. 
Combining equation $\ref{eq:msa}$ and $\ref{eq:mlp}$, we obtain for any index $i$ and $\ell = 1, \cdots, L$
\begin{align*}
    \bm{h}^\ell_i =& \mathrm{MLP}^\ell(\hat{\bm{h}}^\ell)_i + \mathrm{MSA}^\ell(\bm{h}^{\ell-1})_i + \bm{h}^{\ell-1}
\end{align*}
Then, for any $i$ and for any $\ell \in \{0,\cdots,L\}$, we can unroll the equation to decompose $\bm{h}^L$ as
\begin{align*}
    \bm{h}^L_i &=  \bm{h}^{\ell}_i + \sum_{j = \ell+1}^{L} \mathrm{MLP}^j(\hat{\bm{h}}^j)_i + \mathrm{MSA}^j(\bm{h}^{j-1})_i\\
    P \bm{h}^L_i &= P \bm{h}^{\ell}_i + \sum_{j = \ell+1}^{L} P \mathrm{MLP}^j(\hat{\bm{h}}^j)_i + P \mathrm{MSA}^j(\bm{h}^{j-1})_i
\end{align*}
and the output logit of the LLM is   \Chengzhi{Remove exp, talk about logit has one to one mapping, since softmax is also one to one, then finish the prove.}
\begin{align*}\bm{y}_i = \mathrm{softmax}(P \bm{h}^L_i) \propto & \; \mathrm{exp}(P \bm{h}^{\ell}_i) \cdot \prod_{j = \ell+1}^{L}  \exp(P \mathrm{MLP}^j(\hat{\bm{h}}^j) _i) \cdot \\
&\prod_{j = \ell+1}^{L} \exp ( P \mathrm{MSA}^j(\bm{h}^{j-1}) _i)
\end{align*}

For any layer $\ell$ and index $i$, we can decompose output $\bm{y}_i$ into a geometric average of $\exp(P \bm{v})$ for a set of vectors $\bm{v}$. We can understand $\exp(P \bm{v})$ as a prediction about next token distribution based on information contained in $\bm{v}$, and the final prediction $\bm{y}_i = \mathrm{softmax}(P \bm{h}^L_i)$ is an ensemble of predictions with different $\bm{v}$. 

In particular, for any layer $\ell$, $\mathrm{exp}(P \bm{h}^{\ell}_i)$ maps hidden embedding $\bm{h}^{\ell}_i$ on layer $\ell$ to a contribution to the overall prediction about next token distribution based on information contained in $\mathrm{exp}(P \bm{h}^{\ell}_i)$. This mapping will show that embeddings in different layers represent information in a unified way. 


% \Chengzhi{One to One maping from concept to output semantic}



\textbf{Decomposition into layer contribution.} 

\textbf{Embeddings in all layers represent information in a same way} \tony{need more work on polishing this part argument} 

% Each layer contains information that's useful for predicting next token distribution. Each transformer layer understand the information and produce more useful information for understanding. We assume that $\exp(P\bm{v})$ is an identifier of the information represented by $\bm{v}$. This assumption is justified by (1) The distribution of next token is a highly granular space, where any difference in information represented by embedding would decode through $\exp(P\bm{v})$ into a different next token distribution; (2) Hidden embeddings are used by LLMs to understand what next token is, so if two embeddings map to the same output token distribution, the information represented by the two embeddings is indistinguishable for LLMs.  

If we obtain hidden embedding $\bm{h}^{\ell_1}_i = \bm{v}$ on layer $\ell_1$, LLM will decode information it represents into $\mathrm{exp}(P \bm{h}^{\ell_1}_i) = \mathrm{exp}(P \bm{v})$, which is the contribution of next token prediction from layer $\ell_1$. At the same time, if we obtain hidden embedding $\bm{h}^{\ell_2}_i = \bm{v}$ on layer $\ell_2$,  $\bm{h}^{\ell_2}_i$ will contribute to the next token prediction in the same way with $\mathrm{exp}(P \bm{h}^{\ell_2}_i) = \mathrm{exp}(P \bm{h}^{\ell_1}_i) = \mathrm{exp}(P \bm{v})$. Therefore, the information represented by $\bm{v}$ on layer $\ell_1$ is also represented on layer $\ell_2$ by the same vector $\bm{v}$ .

% and we also obtain hidden embedding $\bm{h}^{\ell_2}_i = \bm{v}$ on layer $\ell_2$, the two embeddings decode into a same prediction about next token distribution $\mathrm{exp}(P \bm{h}^{\ell_1}_i) = \mathrm{exp}(P \bm{h}^{\ell_2}_i)$. Therefore, the information represented by $\bm{h}^{\ell_1}_i$ is the same as information represented by $\bm{h}^{\ell_2}_i$.

If we obtain $\bm{h}^{\ell_1}_i = \bm{v}$ and it represent a certain piece of information, the downstream operations on layer $\ell_1$ ($\mathrm{MSA^{\ell_1+1}}$ and $\mathrm{MLP^{\ell_1+1}}$) are trained to recognize the piece of information in the representation of $\bm{v}$ and then process the information. Suppose we obtain $\bm{h}^{\ell_2}_i = \bm{v}$ on layer $\ell_2$ and use it as input to downstream operations on layer $\ell_1$, the downstream operations will identify it as the information represented by $\bm{h}^{\ell_1}_i = \bm{v}$. Since when we obtain $\bm{h}^{\ell_1}_i = \bm{h}^{\ell_2}_i = \bm{v}$ on two different layers, they represent the same information, the downstream operations on layer $\ell_1$ are able to identify and process information in $\bm{h}^{\ell_2}_i$ properly. Therefore, \texttt{SelfIE}'s replacement of hidden embedding on a different layer during the forward pass correctly leverages the trained capability of transformer layers in an LLM.


% When we obtain $\bm{u}$ from layer $\bm{h}^\ell$, $\bm{u}$ represents a unique concept $c$ such that $\bm{u} \in r_{\bm{h}^\ell}(c)$. Then for another layer $\bm{h}^{\ell'}$, $\bm{u} \in r_{\bm{h}^{\ell'}}(c)$ and thus represents the same concept on $\bm{h}^{\ell'}$. Since $f_{\bm{h}^{\ell'}}$ is trained to process $c$ in the representation of vectors in $r_{\bm{h}^{\ell'}}(c)$, $f_{\bm{h}^{\ell'}}$ is able to correctly process the concept represented by $\bm{u}$ by taking $\bm{u}$ as input. 

% $\exp(P \bm{h}^\ell_i)$ and $\exp(P \bm{v})$
% For any $\bm{v} \in \Lambda$, choosing appropriate $\ell$, $\bm{y}_i$ could be decomposed into an expression proportional to geometric mean of $\exp\{P \bm{u}\}$ with $\bm{u} \in G \subset \Lambda$ and $\bm{v} \in G$. 
% }
% In other words, each $\exp(P \bm{v})$ can be viewed as a mapping from each $\bm{u}$ to a prediction of next token based on information in respective vector. $\bm{y}_i$ is a geometric average ensemble predictions with a set of these vectors.
% \begin{definition}
% \label{def:concept}
% A concept $c$ at position $i$ contains semantic information about input $\bm{x}_{<i}$ that could be used to predict what token $i+1$ is. Two concepts $c = c'$ if information from two concepts has the same effects on predicting output token $\bm{y}_i$.
% \end{definition}

% Since producing $\bm{y}_i$ involves $\bm{h}^{\ell}_i, \mathrm{MSA}^\ell(\bm{h}^{\ell})_i, \mathrm{MLP}^\ell(\hat{\bm{h}}^\ell)_i$ for all $\ell$, by Definition \ref{def:concept}, each of $\bm{h}^{\ell}_i, \mathrm{MSA}^\ell(\bm{h}^{\ell})_i, \mathrm{MLP}^\ell(\hat{\bm{h}}^\ell)_i$ represents a concept $c$. For any input $\bm{x}$, if we obtained $\bm{h}^{\ell}_i = \bm{v}$, since $\bm{h}^{\ell}_i$ undergo same operations in the rest of transformer forward pass regardless $\bm{x}$ and affect output $\bm{y}_i$ in the same way, for each $\bm{v}$, there's a unique concept $c$ it represents. We can therefore define a mapping between vector $\bm{v}$ and a concept $c$ on layer $\bm{h}^{\ell}_i$. Similar for $\mathrm{MSA}^\ell(\bm{h}^{\ell})_i, \mathrm{MLP}^\ell(\hat{\bm{h}}^\ell)_i$. We can group all such mapping in one layer to define a concept mapping relationship for the layer. 
% \begin{definition}
%     Given input $\bm{x}$, define layer $A$ as a location where we can obtain an embedding vector $\bm{v} \in \mathbb{R}^{\mathrm{hidden\ dim}}$ at any position in $A$. In particular, we focus on $ \bm{h}^{\ell}$, $\mathrm{MSA}^\ell(\bm{h}^{\ell-1})$, and $\mathrm{MLP}^\ell(\hat{\bm{h}}^{\ell})$. For example, we say we obtain $\bm{v}$ at layer $\bm{h^\ell}$ if $u = \bm{h^\ell}_i$ for any position $i$. Denote the downstream operations that take vectors obtained at $A$ as input as $f_A$.
% \end{definition}

% Transformer in LLM maps natural language to natural language; therefore, the hidden embeddings provides vector representations for semantic information. Denote such information as concept $c$. 
% \begin{definition}
%     The representation relationship on layer $A$ can be formalized by a mapping $r_A: C_A \rightarrow \mathcal{P}(\mathbb{R}^{\mathrm{hidden\ dim}})$ that maps each concept to a set of hidden embeddings that represent the concept in layer $A$: $V_A= r_A(c)$. 
% \end{definition}
% Downstream operations of each layer $f_A$ is trained to process concept $c$ when represented by vectors in $r_A(c)$. 

% \begin{definition}
%         Denote $A$ to be a layer such as $\bm{h}^{\ell}_\cdot$, or $\mathrm{MSA}^\ell(\bm{h}^{\ell})_\cdot$, or $\mathrm{MLP}^\ell(\hat{\bm{h}}^\ell)_\cdot$ for a given $\ell$. The representation relationship on layer $A$ can be formalized by a mapping $r_A: C_A \rightarrow \mathcal{P}(\mathbb{R}^{\mathrm{hidden\ dim}})$ that maps each concept to a set of hidden embeddings that represent the concept in layer $A$: $V_A= r_A(c)$. 
% \end{definition}
% \begin{remark}
%     Note that we group all indices $i$ in each layer $A$ together in one representation mapping $r_A$ since the operations in the rest of transformer are the same for vectors at different positions on the same layer.
% \end{remark}

% \begin{lemma}
% \label{lem:decomposition}
%     Given an input $\bm{x}$, let the set of resulting hidden states at position $i$ be $\Lambda = \{\bm{h}^{\ell}_i\}_{\ell\in\{0\cdots L\}} \cup \{\mathrm{MSA}^\ell(\bm{h}^{\ell})_i\}_{\ell\in \{1\cdots L\}} \cup \{\mathrm{MLP}^\ell(\hat{\bm{h}}^\ell)_i\}_{\ell \in \{1\cdots L\}}$. For any $\bm{v} \in \Lambda$, there exists $G \subset \Lambda$ such that $\bm{y}_i$ is a geometric average of next token distribution predicted separately with information in each element of $G$.
% \end{lemma}
% \begin{proof}
% Combining equation $\ref{eq:msa}$ and $\ref{eq:mlp}$, we obtain for any $i$ and $\ell = 1, \cdots, L$
% \begin{align*}
%     \bm{h}^\ell_i =& \mathrm{MLP}^\ell(\hat{\bm{h}}^\ell)_i + \mathrm{MSA}^\ell(\bm{h}^{\ell-1})_i + \bm{h}^{\ell-1}
% \end{align*}
% Then, for any $i$ and for any $\ell \in \{0,\cdots,L\}$, we can unroll the equation to decompose $\bm{h}^L$ as
% \begin{gather*}
%     \bm{h}^L_i =  \bm{h}^{\ell}_i + \sum_{j = \ell+1}^{L} \mathrm{MLP}^j(\hat{\bm{h}}^j)_i + \mathrm{MSA}^j(\bm{h}^{j-1})_i\\
%     P \bm{h}^L_i = P \bm{h}^{\ell}_i + \sum_{j = \ell+1}^{L} P \mathrm{MLP}^j(\hat{\bm{h}}^j)_i + P \mathrm{MSA}^j(\bm{h}^{j-1})_i\\
%     \mathrm{softmax}(P \bm{h}^L_i) \propto\mathrm{exp}(P \bm{h}^{\ell}_i)   \cdot \prod_{j = \ell+1}^{L}  \exp ( P \mathrm{MLP}^j(\hat{\bm{h}}^j) _i) \\ \cdot \prod_{j = \ell+1}^{L} \exp ( P \mathrm{MSA}^j(\bm{h}^{j-1}) _i)
% \end{gather*}

% For any $\bm{v} \in \Lambda$, choosing appropriate $\ell$, $\bm{y}_i$ could be decomposed into an expression proportional to geometric mean of $\exp\{P \bm{u}\}$ with $\bm{u} \in G \subset \Lambda$ and $\bm{v} \in G$. 
% \end{proof}
% In other words, each $\exp(P \bm{v})$ can be viewed as a mapping from each $\bm{u}$ to a prediction of next token based on information in respective vector. $\bm{y}_i$ is a geometric average ensemble predictions with a set of these vectors.
% \begin{assumption}
%     $\exp(P\bm{v})$ is a unique identifier of the concept represented by $\bm{v}$. 
% \end{assumption}
% This assumption is justified by (1) LLMs are trained to predict the next token, so the concept represented by hidden embeddings is predominately associated with predicting next token; (2) the distribution of next token is a highly granular space, where any difference in concept represented by embedding would decode through $\exp(P\bm{v})$ into a different next token distribution. 


% Since the operation $\exp(P \bm{v})$ can be decomposed into operation on each position of $\bm{v}$, we will focus on the embedding space that contains individual position vectors $\bm{v}_i$. The subscript doesn't denote for a specific position since operations on each $\bm{v}_i$ is same at all positions. Each $\bm{v}_i$ is mapped to a prediction of next token at position $i$. By Definition \ref{def:concept} each $\bm{v}_i$ represents a semantic concept $c_{\bm{v_i}}$. 
 

% \begin{assumption}
%     $\bm{H}^\ell = \bm{H}^{\ell'} = \bm{H}$ for all $\ell, \ell' \in \{0,1\cdots,L\}$. We justify the assumption by (1) observing that $\bm{H}^\ell, \bm{H}^{\ell'}$ are bounded to the same region because of LayerNorm in MLP and MSA; (2) Each embedding space is dense. 
% \end{assumption}

% \begin{assumption}
%     $P$ is full column rank. This can be easily verified by inspecting trained model parameter. This assumption implies that $\bm{y}_i = P \bm{h}^\ell_i$ is an injective mapping.
% \end{assumption}

% \begin{corollary}
%     Since each $v \in \Lambda$ contains semantic information that predicts next token at position $i$, $\bm{h}_i^{\ell}$ provides vector representation for a concept $c$. The space of $\{\bm{h}^{\ell}_i\}$ provides representation for $\bm{h}^{\ell}_i$ a set of concept $C^\ell$. Similarly, space $\{\mathrm{MSA}^\ell(\bm{h}^{\ell})_i\}$ represents $C^\ell_{\mathrm{MSA}}$, and space $\{\mathrm{MLP}^\ell(\hat{\bm{h}}^\ell)_i\}$ represents $C^\ell_{\mathrm{MSA}}$. For embedding space $A$, denote the corresponding set of concepts represented as $C_A$. Note that each set $A$ contains embedding at all positions $i$ since application of MLP and MSA is same at all positions. Index $i$ only serves to denote the space contain single position vectors.
% \end{corollary}

% \begin{lemma}
%     Given concept $c$ and a layer $A$, for all $\bm{v},\bm{v}'$ in $V_A= r_A(c)$, $\exp(P \bm{v}) = \exp(P \bm{v}')$.  
% \end{lemma}
% \begin{proof}
%     Assume otherwise, $\bm{v}$ and $\bm{v}'$ results in different prediction about next token with $\exp(P \bm{v}) \ne \exp(P \bm{v}')$ and thus represent different semantic concepts. Contradiction.
% \end{proof}
% \begin{definition}
%     Define mapping $f_A: C \rightarrow \mathbb{R}^M$ as $f_A(c) = \exp(Pv)$ for any $\bm{v} \in r_A(c)$.
% \end{definition}
% \begin{lemma}
% \label{lem:unique}
%     If $c \ne c'$, $r_A(c) \cap r_A(c') = \emptyset$. In other words, there exists an injective mapping from vector to cocnept  
% \end{lemma}
% \begin{proof}
%     Assume otherwise, there exists $c,c' \in C_A$ such that $c \ne c'$ and $\bm{v} \in r^\ell(c)$ and $\bm{v} \in r^\ell(c')$, then $f^\ell(c) = f^\ell(c)$. In other words, based on semantic information in concept $c,c'$, we reach same prediction about next token distribution. This contradicts definition of equivalence between concepts. Similar proof for MSA and MLP.
% \end{proof}
% \begin{theorem}
%     The representation of concepts is consistent in all layers. In other words, there exists universal set of concept $C$ and representation mapping $r$ such that for any layer $A$, $C = C_A$, and $r$ is the same mapping as $r_A$.
% \end{theorem}
% \begin{proof}
%     Let $\bm{u} \in \mathbb{R}^{\mathrm{hidden\ dim}}$. Since predicted next token distribution $\exp(P\bm{u})$ is irrelevant to on which layer we obtain $\bm{u}$,  the concept represented by $\bm{u}$ is same regardless from which layer we obtain $\bm{u}$. Therefore, let $A, A'$ be two layers, if $u \in r_{A}(c)$, then $u \in r_A'(c)$, and $c \in C_A, C_{A'}$. 
% \end{proof}
% \begin{definition}
%     By Lemma $\ref{lem:unique}$, we can define an inverse representation mapping as $\bar{r}(\bm{v}) = c$ if $\bm{v} \in r(c)$.
% \end{definition}
% % \begin{lemma}
% %     If $\bm{u} = \sum_i v_i$ and $\bm{u} = r(c)$ for some $c \in C$. Then $v_i = r(c_i)$ for some $c_i$.
% % \end{lemma}
% % \begin{proof}
% %     Similar to proof for lemma \ref{lem:decomposition}.
% % \end{proof}
% \begin{definition}
%     If $c = \bar{r}(\bm{u})$ and $c_i = \bar{r}(v_i)$, for some functions $\bm{u} = f(u_1,u_2,\cdots)$, we define corresponding operation on concepts $\bar{f}$ as $c = \bar{f}(c_1, c_2, \cdots)$.
% \end{definition}
% When transformer a forward pass operation $f$ described in Equations \ref{eq:msa}, \ref{eq:mlp} (MSA, MLP, and addition of residuals) maps vectors $v_1 \in A$ to $v_2 \in B$, we can interpret the operation with the corresponding operation on concepts $\bar{f}$ that maps the concept $\bar{r}(v_1)$ to $\bar{r}(v_2)$, and the vector that represents $\bar{r}(v_2)$ in $A$ is also $v_2$. A transformer is therefore a sequence of concept conversion, where relationship between concepts and vectors representing them is same in all layers. 

% Then, for example, when applying $\mathrm{MSA}^\ell(\bar{\bm{h}}^{\ell-1})+ \bar{\bm{h}}^{\ell-1}$ in Equation \ref{eq:surgery-msa} while replacing $\bar{\bm{h}}^\ell_i =& \bm{h}^{\ell^*}_{i^*}$ and $\ell \ne \ell^*$, the operation attains the desired purpose of obtaining a new vector that represents MSA's combination of $\bar{r}(\bm{h}^{\ell^*}_{i^*})$ and concepts represented by other vectors on the same layer. \texttt{SelfIE}'s replacement of embedding on different layers therefore leverages this inherent characteristic of transformer representation space and produce meaningful outputs.
% When we obtain $\bm{u}$ from layer $\bm{h}^\ell$, $\bm{u}$ represents a unique concept $c$ such that $\bm{u} \in r_{\bm{h}^\ell}(c)$. Then for another layer $\bm{h}^{\ell'}$, $\bm{u} \in r_{\bm{h}^{\ell'}}(c)$ and thus represents the same concept on $\bm{h}^{\ell'}$. Since $f_{\bm{h}^{\ell'}}$ is trained to process $c$ in the representation of vectors in $r_{\bm{h}^{\ell'}}(c)$, $f_{\bm{h}^{\ell'}}$ is able to correctly process the concept represented by $\bm{u}$ by taking $\bm{u}$ as input. Therefore, \texttt{SelfIE}'s replacement of hidden embedding on a different layer during the forward pass correctly leverages the trained capability of transformer layers in an LLM.
% Given a layer $A$ and all operations involved in converting $\bm{u}$ on layer $A$ to final output $\mathbm{y}_i$ (let vectors at other position on layer $A$ as given part of the operations for MSA). Let the aggregation of the operation be $f$. $f$ is trained to decode the concept represented by $\bm{u}$ into next token prediction $\bm{y}_i$. 

% \subsection{Choosing replacement layer $k$}
% We have shown that the transformer is able to decode information in the embedding to interpret that we select from layer $\ell^*$ when we replace it into a different layer $k$ during step \ref{eq:replace} in the interpretation forward pass. How do we choose which layer $k$ to conduct the replacement? \cv{Need to clarify that this is the layer you inject into the interpretation LLM. You can interpret any layer K, but you need to decide where to put it in the second LLM for interpetation. This is confusing, and we should setup terminology so it's clear. We might want to create a consistent name for the two LLMs.... original LLM and interpretable LLM? We need a way to talk about the two different LLMs.} We hypothesize that two model behaviors might result in conflicting selection criteria for $k$ to obtain optimal interpretation quality. We provide a framework to measure the two behaviors quantitatively and select $k$ in experiments by finding the equilibrium between minimizing the adverse effects from each model behavior.

% \tony{condense these two as short arguments in ablation over different k with textworld in ablation}
% \textbf{Information distribution shift} Although every transformer layer share a same representation mapping, each transformer layer might have seen a different distribution of information at training time since each layer is applied strictly sequentially. For example, early layers might be trained with more word-level concepts, and late layers might be trained with more complex concepts. Because of the distribution shift, we hypothesize that \texttt{SelfIE} results in better explanations when $k$ is closed to $\ell^*$. Since we assumed that $\exp(P(\bm{v}))$ characterizes the information represented by $v$, we use average output distribution given embeddings of one layer $p_\ell := \mathbb{E}_{\bm{h}_i^{\ell}}\left[\mathrm{softmax}(P \bm{h}_i^{\ell})\right] \propto \mathbb{E}_{\bm{h}_i^{\ell}}\left[\exp(P \bm{h}_i^{\ell})\right] $ as a proxy of characterizing the distribution of information represented in layer $\ell$. We measure the distribution difference between layer $k$ and layer $\ell^*$ with $D_{KL}(p_k || p_{\ell^*})$.

% \textbf{Effective Information Blending} At the same time, if $\ell$ is too large, the lack of MSA operations might prevent information in $\bm{h}_{i^*}^{\ell^*}$ from flowing into the last position that decides output. The last position embedding might also prematurely blend in too much information about the placeholder tokens in interpretation prompt. Therefore, we hypothesize that explanation quality is higher when $\ell$ is smaller. Ideally, different $\bm{h}_{i^*}^{\ell^*}$ should result in different text explanations. At extreme, if all replacement is done on last layer, resulting text explanation would be same for all $\bm{h}_{i^*}^{\ell^*}$. Therefore, we measure effectiveness of information blending with a given $k$ with $H(\mathbb{E}_{\bm{h}_{i^*}^{\ell^*}}[\hat{\bm{y}} | k])$ where $H$ is information entropy.


% \begin{remark}
%     $r^\ell$ is injective. 
% \end{remark}
% \begin{definition}
%     If a $\bm{h}^\ell_i$ contains information that $P\bm{h}^\ell_i $can decode into meaningful next token prediction, each $\bm{h}^\ell_i$ represents meaningful semantic concepts that allows for such prediction. Let $C^\ell$ be the set of all concepts that could be represented by embedding on layer $\ell$, there exists a mapping $r^\ell: C^\ell \rightarrow \mathcal{P}(\mathbb{R}^{\textrm{hidden dim}})$ that maps each concept to a set of hidden embedding that represents the concept $\bm{v}^\ell= r^\ell(c)$. Note that $\bm{y} = P r^\ell(c)$ maps concept $c$ to prediction $\bm{y}$.
% \end{definition}
% \begin{definition}
%     $c = c'$ for $c,c' \in C^\ell$ if $P r^\ell(c).= P r^\ell(c')$. 
% \end{definition}





\texttt{SelfIE} will place embeddings from layer $\ell^*$ to layer $k$ during interpretation.
A fundamental premise of this process is the consistent representation of information across different layers, a characteristic inherent to the architecture of transformers due to their residual connections.


% which requires different layers to represent the same information in the same way. We will show that this is inherently achieved because of the residual connection in transformer architecture.


% In the interpretation forward pass of \texttt{SelfIE} interpretation procedure, we replace the placeholder hidden embedding $\hat{\bm{h}^k_s}$ at layer $k$ with the embedding being interpreted $\bm{h}^{\ell^*}_{i^*}$ from layer $\ell^*$ in the original pass. The layer $\ell^*$ that $\bm{h}^{\ell^*}_{i^*}$ comes from in original forward pass can be different from layer $k$ that we place the embedding in during interpretation pass. In order for interpretation forward pass to correctly process information in $\bm{h}^{\ell^*}_{i^*}$, different layers need to represent a same information in the same way. We will show that this is inherently achieved because of the residual connection in transformer architecture.

% We will show by decomposing the relationship between output $\bm{y}$ and $\bm{h}^{\ell}$ on different layers $\ell$ that a same vector on different layer represents a same concept; thus choosing to replace on a different layer correctly leverages trained functionality of each transformer layer and produces meaningful outputs.


% \Chengzhi{One to One maping from latent to output semantic}

% \begin{assumption}
        Let $P$ be the final matrix in the LLM transformer. $P$ converts latent tokens into output logits. We empirically observe that $P$ is an injective function, mapping distinct input vectors to distinct outputs. 
        % \tony{This assumption can be easily verified by examining rank of trained projection matrix of a transformer. But this assumption is not necessary?}
% \end{assumption}

% \begin{assumption}
       We posit that a well-trained Language Model (LLM) generates a unique output for each input vector, provided these vectors are semantically equivalent.
% \end{assumption}
 This is because based on the expectation of consistent performance from a mature LLM that has been adequately trained.

% The assumptions hold when LLM has been trained to produce accurate output for each query.
% In the following, we will show that if the transformer based LLM has been trained to converge such that it will not produce different output probability vector (before sampling) for same information, then we can place embeddings from one latent layer to another one.

Our key observation is that the output vector in a transformer can be conceptualized as a linear combination of latent embeddings. Mathematically, this is represented as:
\begin{align*}
    \bm{o}^\ell_i = P \sum_1^L \lambda_i \h_i + P \sum_1^L \lambda'_j \mathrm{MLP}^i(\bm{h}^{j-1})_i
\end{align*}
% \begin{align*}
%     \bm{h}^L_i &=  \bm{h}^{\ell}_i + \sum_{j = \ell+1}^{L} \mathrm{MLP}^j(\hat{\bm{h}}^j)_i + \mathrm{MSA}^j(\bm{h}^{j-1})_i\\
%     =& \bm{h}^{\ell}_i + \sum_{j = \ell+1}^{L} \mathrm{MLP}^j(\hat{\bm{h}}^j)_i  +\sum_{j = \ell+1}^{L} \sum_{i'=1}^N a_{ii'}^j  (\bm{h}^{j-1}_{i'})_i\\
%     &=  \sum_{j=\ell}^{L} \bm{h}^{j}_i +\sum_{j = \ell+1}^{L} \sum_{i'=1}^N a_{ii'}^j  \bm{h}^{j-1}_{i'} \\
%     \intertext{Where $a_ii'$ is the attention weight between token $i$ and $i'$ on layer $j$. Choose $\ell=1$}
%     \bm{h}^L_i &=  \sum_{j=1}^{L} \bm{h}^{j}_i +\sum_{j = 1}^{L-1} \sum_{i'=1}^N a_{ii'}  \bm{h}^{j}_{i'} \\
%     P \bm{h}^L_i &= P \bm{h}^{\ell}_i + \sum_{j = \ell+1}^{L} P \mathrm{MLP}^j(\hat{\bm{h}}^j)_i + P \mathrm{MSA}^j(\bm{h}^{j-1})_i
% \end{align*}
where $\bm{o}^\ell_i$ denotes the output vector at layer $\ell$, $\lambda_i$ are the coefficients in the linear combination, and $\h_i$ are the latent embeddings.

% \begin{proposition}
Thus, in a transformer-based LLM, the output probability vector $\bm{o}$, computed before sampling, will remain constant for a given latent embedding vector $\h_i$, irrespective of the layer from which this embedding originates.
% \end{proposition}
The semantic representation of $\h_i$, obtained through the transformation $P \h_i$, mandates a consistent informational representation. In other words, varying representations of the same information would lead to different output vectors. 
% Given that the semantic of the latent $\h_i$ can be calculated by performing $P \h_i$, $h_i$ needs to represent the same information in the same way, because otherwise, if the same information is represented into different vectors, then they will be mapped to different output vectors. 



% \begin{lemma}
% For any output concept represented by a output vector $t$, there exists a unique embedding $h$ in the latent space of a transformer that maps to it.
% \end{lemma}


\begin{assumption}
        For a given concept $C$ encoded by the LLM, there exists a unique corresponding output vector $\bm{o}$. 
\end{assumption}
This assumption typically holds for a well-converged language model, where identical semantic inputs yield identical outputs.


% \Chengzhi{One to One maping from latent to output semantic}

\begin{theorem}[\textbf{Shared Embeddings}]
In the above transformer model, all latent layers represent the same concept $C$ using identical embedding vectors.
\end{theorem}

The essence of this theorem lies in the unique representation of concepts: if each concept corresponds to a unique output vector, and each output vector relates to a unique latent vector, then it follows that identical latent representations across layers signify the same concept. \texttt{SelfIE} leverage this insight to interchange embeddings between layers during interpretation, where we also demonstrate the effectiveness through empirical results.

% If there is a unique latent vector for each output vector, and each concept is uniquely represented by a unique output vector, then all the latent representations that has the same value will share the same concept. This explains why our algorithm can paste embeddings from one latent layer to another one during interpertation.


% We denote the output logit to be $o$. Because of the residual connection in transformer, we can write $o$ as a linear combination of the latent embeddings in the input.
